Competitive Sequential Screening

We study competition between firms that contract with consumers before the consumers fully learn their product preferences. In a Hotelling duopoly, firms screen consumers by offering menus of option contracts. We characterize the unique equilibrium. Consumers select contracts from both firms. Each consumer is endogenously locked into the firm from which he chooses an option with a lower strike price. Lock-in yields inefficient consumption. Yet earlier contracting stiffens competition because less informed consumers are more homogeneous. Sufficiently early contracting raises consumer surplus relative to spot pricing -- reversing the ranking under monopoly. Exclusive contracting further increases consumer surplus by intensifying competition.

==> Duopoly.tex <==
% two columns: x y (pgfplots)
-0.990000000000 5.989264059509
-0.980000000000 5.979295337645
-0.970000000000 5.969329795410
-0.960000000000 5.959367724377
-0.950000000000 5.949409439450
-0.940000000000 5.939455280386
-0.930000000000 5.929505613388
-0.920000000000 5.919560832759
-0.910000000000 5.909621362638
-0.900000000000 5.899687658785
-0.890000000000 5.889760210442
-0.880000000000 5.879839542259
-0.870000000000 5.869926216279
-0.860000000000 5.860020833980
-0.850000000000 5.850124038388
-0.840000000000 5.840236516231
-0.830000000000 5.830359000147
-0.820000000000 5.820492270949
-0.810000000000 5.810637159916
-0.800000000000 5.800794551138
-0.790000000000 5.790965383875
-0.780000000000 5.781150654954
-0.770000000000 5.771351421178
-0.760000000000 5.761568801743
-0.750000000000 5.751803980662
-0.740000000000 5.742058209174
-0.730000000000 5.732332808144
-0.720000000000 5.722629170430
-0.710000000000 5.712948763214
-0.700000000000 5.703293130286
-0.690000000000 5.693663894265
-0.680000000000 5.684062758746
-0.670000000000 5.674491510365
-0.660000000000 5.664952020759
-0.650000000000 5.655446248422
-0.640000000000 5.645976240423
-0.630000000000 5.636544133996
-0.620000000000 5.627152157963
-0.610000000000 5.617802633994
-0.600000000000 5.608497977686
-0.590000000000 5.599240699430
-0.580000000000 5.590033405079
-0.570000000000 5.580878796381
-0.560000000000 5.571779671168
-0.550000000000 5.562738923293
-0.540000000000 5.553759542299
-0.530000000000 5.544844612801
-0.520000000000 5.535997313575
-0.510000000000 5.527220916348
-0.500000000000 5.518518784262
-0.490000000000 5.509894370018
-0.480000000000 5.501351213684
-0.470000000000 5.492892940163
-0.460000000000 5.484523256307
-0.450000000000 5.476245947688
-0.440000000000 5.468064875001
-0.430000000000 5.459983970115
-0.420000000000 5.452007231764
-0.410000000000 5.444138720879
-0.400000000000 5.436382555565
-0.390000000000 5.428742905729
-0.380000000000 5.421223987358
-0.370000000000 5.413830056468
-0.360000000000 5.406565402725
-0.350000000000 5.399434342747
-0.340000000000 5.392441213114
-0.330000000000 5.385590363082
-0.320000000000 5.378886147041
-0.310000000000 5.372332916716
-0.300000000000 5.365935013145
-0.290000000000 5.359696758449
-0.280000000000 5.353622447421
-0.270000000000 5.347716338966
-0.260000000000 5.341982647402
-0.250000000000 5.336425533669
-0.240000000000 5.331049096467
-0.230000000000 5.325857363349
-0.220000000000 5.320854281813
-0.210000000000 5.316043710410
-0.200000000000 5.311429409915
-0.190000000000 5.307015034586
-0.180000000000 5.302804123543
-0.170000000000 5.298800092309
-0.160000000000 5.295006224540
-0.150000000000 5.291425663975
-0.140000000000 5.288061406651
-0.130000000000 5.284916293394
-0.120000000000 5.281993002642
-0.110000000000 5.279294043608
-0.100000000000 5.276821749832
-0.090000000000 5.274578273129
-0.080000000000 5.272565577976
-0.070000000000 5.270785436355
-0.060000000000 5.269239423076
-0.050000000000 5.267928911596
-0.040000000000 5.266855070365
-0.030000000000 5.266018859695
-0.020000000000 5.265421029191
-0.010000000000 5.265062115730
0.000000000000 5.264942442022
0.010000000000 5.265062115730
0.020000000000 5.265421029191
0.030000000000 5.266018859695
0.040000000000 5.266855070365
0.050000000000 5.267928911596
0.060000000000 5.269239423076
0.070000000000 5.270785436355
0.080000000000 5.272565577976
0.090000000000 5.274578273129
0.100000000000 5.276821749832
0.110000000000 5.279294043608
0.120000000000 5.281993002642
0.130000000000 5.284916293394
0.140000000000 5.288061406651
0.150000000000 5.291425663975
0.160000000000 5.295006224540
0.170000000000 5.298800092309
0.180000000000 5.302804123543
0.190000000000 5.307015034586
0.200000000000 5.311429409915
0.210000000000 5.316043710410
0.220000000000 5.320854281813
0.230000000000 5.325857363349
0.240000000000 5.331049096467
0.250000000000 5.336425533669
0.260000000000 5.341982647402
0.270000000000 5.347716338952
0.280000000000 5.353622447421
0.290000000000 5.359696758449
0.300000000000 5.365935013145
0.310000000000 5.372332916716
0.320000000000 5.378886147041
0.330000000000 5.385590363082
0.340000000000 5.392441213114
0.350000000000 5.399434342747
0.360000000000 5.406565402725
0.370000000000 5.413830056468
0.380000000000 5.421223987358
0.390000000000 5.428742905729
0.400000000000 5.436382555565
0.410000000000 5.444138720879
0.420000000000 5.452007231764
0.430000000000 5.459983970115
0.440000000000 5.468064875001
0.450000000000 5.476245947688
0.460000000000 5.484523256307
0.470000000000 5.492892940163
0.480000000000 5.501351213684
0.490000000000 5.509894370018
0.500000000000 5.518518784262
0.510000000000 5.527220916348
0.520000000000 5.535997313575
0.530000000000 5.544844612801
0.540000000000 5.553759542299
0.550000000000 5.562738923293
0.560000000000 5.571779671168
0.570000000000 5.580878796381
0.580000000000 5.590033405079
0.590000000000 5.599240699430
0.600000000000 5.608497977686
0.610000000000 5.617802633994
0.620000000000 5.627152157963
0.630000000000 5.636544133996
0.640000000000 5.645976240423
0.650000000000 5.655446248422
0.660000000000 5.664952020759
0.670000000000 5.674491510365
0.680000000000 5.684062758746
0.690000000000 5.693663894265
0.700000000000 5.703293130286
0.710000000000 5.712948763214
0.720000000000 5.722629170430
0.730000000000 5.732332808144
0.740000000000 5.742058209174
0.750000000000 5.751803980662
0.760000000000 5.761568801743
0.770000000000 5.771351421178
0.780000000000 5.781150654954
0.790000000000 5.790965383875
0.800000000000 5.800794551138
0.810000000000 5.810637159916
0.820000000000 5.820492270949
0.830000000000 5.830359000147
0.840000000000 5.840236516231
0.850000000000 5.850124038388
0.860000000000 5.860020833980
0.870000000000 5.869926216279
0.880000000000 5.879839542259
0.890000000000 5.889760210442
0.900000000000 5.899687658785
0.910000000000 5.909621362638
0.920000000000 5.919560832759
0.930000000000 5.929505613388
0.940000000000 5.939455280386
0.950000000000 5.949409439450
0.960000000000 5.959367724377
0.970000000000 5.969329795410
0.980000000000 5.979295337645
0.990000000000 5.989264059509


==> Exclusive.tex <==
% two columns: x y (pgfplots)
-0.990000000000 6.490000000080
-0.980000000000 6.480000000080
-0.970000000000 6.470000000080
-0.960000000000 6.460000000080
-0.950000000000 6.450000000080
-0.940000000000 6.440000000080
-0.930000000000 6.430000000080
-0.920000000000 6.420000000080
-0.910000000000 6.410000000080
-0.900000000000 6.400000000080
-0.890000000000 6.390000000080
-0.880000000000 6.380000000080
-0.870000000000 6.370000000080
-0.860000000000 6.360000000080
-0.850000000000 6.350000000080
-0.840000000000 6.340000000080
-0.830000000000 6.330000000080
-0.820000000000 6.320000000080
-0.810000000000 6.310000000080
-0.800000000000 6.300000000080
-0.790000000000 6.290000000080
-0.780000000000 6.280000000080
-0.770000000000 6.270000000080
-0.760000000000 6.260000000080
-0.750000000000 6.250000000080
-0.740000000000 6.240000000080
-0.730000000000 6.230000000080
-0.720000000000 6.220000000080
-0.710000000000 6.210000000080
-0.700000000000 6.200000000080
-0.690000000000 6.190000000080
-0.680000000000 6.180000000080
-0.670000000000 6.170000000080
-0.660000000000 6.160000000080
-0.650000000000 6.150000000080
-0.640000000000 6.140000000080
-0.630000000000 6.130000000080
-0.620000000000 6.120000000080
-0.610000000000 6.110000000080
-0.600000000000 6.100000000080
-0.590000000000 6.090000000080
-0.580000000000 6.080000000080
-0.570000000000 6.070000000081
-0.560000000000 6.060000000081
-0.550000000000 6.050000000081
-0.540000000000 6.040000000081
-0.530000000000 6.030000000081
-0.520000000000 6.020000000081
-0.510000000000 6.010000000081
-0.500000000000 6.000000000081
-0.490000000000 5.990000000081
-0.480000000000 5.980000000081
-0.470000000000 5.970000000081
-0.460000000000 5.960000000081
-0.450000000000 5.950000000081
-0.440000000000 5.940000000081
-0.430000000000 5.930000000081
-0.420000000000 5.920000000081
-0.410000000000 5.910000000081
-0.400000000000 5.900000000081
-0.390000000000 5.890000000081
-0.380000000000 5.880000000081
-0.370000000000 5.870000000081
-0.360000000000 5.860000000081
-0.350000000000 5.850000000081
-0.340000000000 5.840000000081
-0.330000000000 5.830000000081
-0.320000000000 5.820000000082
-0.310000000000 5.810000000082
-0.300000000000 5.800000000082
-0.290000000000 5.790000000082
-0.280000000000 5.780000000082
-0.270000000000 5.770000000083
-0.260000000000 5.760000000083
-0.250000000000 5.750000000083
-0.240000000000 5.740000000084
-0.230000000000 5.730000000084
-0.220000000000 5.720000000085
-0.210000000000 5.710000000086
-0.200000000000 5.700000000086
-0.190000000000 5.690000000087
-0.180000000000 5.680000000088
-0.170000000000 5.670000000089
-0.160000000000 5.660000000090
-0.150000000000 5.650000000092
-0.140000000000 5.640000000093
-0.130000000000 5.630000000095
-0.120000000000 5.620000000097
-0.110000000000 5.610000000100
-0.100000000000 5.600000000102
-0.090000000000 5.590000000105
-0.080000000000 5.580000000109
-0.070000000000 5.570000000112
-0.060000000000 5.560000000117
-0.050000000000 5.550000000122
-0.040000000000 5.540000000128
-0.030000000000 5.530000000134
-0.020000000000 5.520000000141
-0.010000000000 5.510000000149
0.000000000000 5.500000000159
0.010000000000 5.510000000149
0.020000000000 5.520000000141
0.030000000000 5.530000000134
0.040000000000 5.540000000128
0.050000000000 5.550000000122
0.060000000000 5.560000000117
0.070000000000 5.570000000112
0.080000000000 5.580000000109
0.090000000000 5.590000000105
0.100000000000 5.600000000102
0.110000000000 5.610000000100
0.120000000000 5.620000000097
0.130000000000 5.630000000095
0.140000000000 5.640000000093
0.150000000000 5.650000000092
0.160000000000 5.660000000090
0.170000000000 5.670000000089
0.180000000000 5.680000000088
0.190000000000 5.690000000087
0.200000000000 5.700000000086
0.210000000000 5.710000000086
0.220000000000 5.720000000085
0.230000000000 5.730000000084
0.240000000000 5.740000000084
0.250000000000 5.750000000083
0.260000000000 5.760000000083
0.270000000000 5.770000000083
0.280000000000 5.780000000082
0.290000000000 5.790000000082
0.300000000000 5.800000000082
0.310000000000 5.810000000082
0.320000000000 5.820000000082
0.330000000000 5.830000000081
0.340000000000 5.840000000081
0.350000000000 5.850000000081
0.360000000000 5.860000000081
0.370000000000 5.870000000081
0.380000000000 5.880000000081
0.390000000000 5.890000000081
0.400000000000 5.900000000081
0.410000000000 5.910000000081
0.420000000000 5.920000000081
0.430000000000 5.930000000081
0.440000000000 5.940000000081
0.450000000000 5.950000000081
0.460000000000 5.960000000081
0.470000000000 5.970000000081
0.480000000000 5.980000000081
0.490000000000 5.990000000081
0.500000000000 6.000000000081
0.510000000000 6.010000000081
0.520000000000 6.020000000081
0.530000000000 6.030000000081
0.540000000000 6.040000000081
0.550000000000 6.050000000081
0.560000000000 6.060000000081
0.570000000000 6.070000000081
0.580000000000 6.080000000080
0.590000000000 6.090000000080
0.600000000000 6.100000000080
0.610000000000 6.110000000080
0.620000000000 6.120000000080
0.630000000000 6.130000000080
0.640000000000 6.140000000080
0.650000000000 6.150000000080
0.660000000000 6.160000000080
0.670000000000 6.170000000080
0.680000000000 6.180000000080
0.690000000000 6.190000000080
0.700000000000 6.200000000080
0.710000000000 6.210000000080
0.720000000000 6.220000000080
0.730000000000 6.230000000080
0.740000000000 6.240000000080
0.750000000000 6.250000000080
0.760000000000 6.260000000080
0.770000000000 6.270000000080
0.780000000000 6.280000000080
0.790000000000 6.290000000080
0.800000000000 6.300000000080
0.810000000000 6.310000000080
0.820000000000 6.320000000080
0.830000000000 6.330000000080
0.840000000000 6.340000000080
0.850000000000 6.350000000080
0.860000000000 6.360000000080
0.870000000000 6.370000000080
0.880000000000 6.380000000080
0.890000000000 6.390000000080
0.900000000000 6.400000000080
0.910000000000 6.410000000080
0.920000000000 6.420000000080
0.930000000000 6.430000000080
0.940000000000 6.440000000080
0.950000000000 6.450000000080
0.960000000000 6.460000000080
0.970000000000 6.470000000080
0.980000000000 6.480000000080
0.990000000000 6.490000000080


==> Spot.tex <==
% two columns: x y (pgfplots)
-0.990000000000 5.230238777408
-0.980000000000 5.223485038260
-0.970000000000 5.216780660992
-0.960000000000 5.210126129226
-0.950000000000 5.203521926292
-0.940000000000 5.196968535125
-0.930000000000 5.190466438163
-0.920000000000 5.184016117248
-0.910000000000 5.177618053522
-0.900000000000 5.171272727251
-0.890000000000 5.164980618065
-0.880000000000 5.158742204266
-0.870000000000 5.152557963160
-0.860000000000 5.146428370829
-0.850000000000 5.140353902028
-0.840000000000 5.134335030075
-0.830000000000 5.128372226747
-0.820000000000 5.122465962172
-0.810000000000 5.116616704710
-0.800000000000 5.110824920862
-0.790000000000 5.105091075151
-0.780000000000 5.099415630013
-0.770000000000 5.093799045688
-0.760000000000 5.088241780114
-0.750000000000 5.082744288810
-0.740000000000 5.077307024773
-0.730000000000 5.071930438364
-0.720000000000 5.066614977199
-0.710000000000 5.061361086039
-0.700000000000 5.056169206680
-0.690000000000 5.051039777842
-0.680000000000 5.045973235061
-0.670000000000 5.040970010578
-0.660000000000 5.036030533229
-0.650000000000 5.031155228340
-0.640000000000 5.026344517612
-0.630000000000 5.021598819017
-0.620000000000 5.016918546688
-0.610000000000 5.012304110814
-0.600000000000 5.007755917529
-0.590000000000 5.003274368783
-0.580000000000 4.998859862341
-0.570000000000 4.994512791514
-0.560000000000 4.990233545168
-0.550000000000 4.986022507590
-0.540000000000 4.981880058384
-0.530000000000 4.977806572371
-0.520000000000 4.973802419487
-0.510000000000 4.969867964682
-0.500000000000 4.966003567821
-0.490000000000 4.962209583585
-0.480000000000 4.958486361375
-0.470000000000 4.954834245189
-0.460000000000 4.951253573632
-0.450000000000 4.947744679660
-0.440000000000 4.944307890603
-0.430000000000 4.940943528045
-0.420000000000 4.937651907702
-0.410000000000 4.934433339393
-0.400000000000 4.931288126898
-0.390000000000 4.928216567925
-0.380000000000 4.925218953967
-0.370000000000 4.922295570255
-0.360000000000 4.919446695671
-0.350000000000 4.916672602670
-0.340000000000 4.913973557184
-0.330000000000 4.911349818575
-0.320000000000 4.908801639541
-0.310000000000 4.906329266045
-0.300000000000 4.903932937252
-0.290000000000 4.901612885438
-0.280000000000 4.899369335954
-0.270000000000 4.897202507140
-0.260000000000 4.895112610264
-0.250000000000 4.893099849462
-0.240000000000 4.891164421680
-0.230000000000 4.889306516611
-0.220000000000 4.887526316647
-0.210000000000 4.885823996817
-0.200000000000 4.884199724740
-0.190000000000 4.882653660577
-0.180000000000 4.881185956978
-0.170000000000 4.879796759043
-0.160000000000 4.878486204275
-0.150000000000 4.877254422539
-0.140000000000 4.876101536027
-0.130000000000 4.875027659218
-0.120000000000 4.874032898845
-0.110000000000 4.873117353863
-0.100000000000 4.872281115422
-0.090000000000 4.871524266835
-0.080000000000 4.870846883557
-0.070000000000 4.870249033163
-0.060000000000 4.869730775322
-0.050000000000 4.869292161785
-0.040000000000 4.868933236369
-0.030000000000 4.868653942275
-0.020000000000 4.868454490179
-0.010000000000 4.868334809934
0.000000000000 4.868295013817
0.010000000000 4.868334809934
0.020000000000 4.868454490179
0.030000000000 4.868653942275
0.040000000000 4.868933236369
0.050000000000 4.869292161785
0.060000000000 4.869730775322
0.070000000000 4.870249033163
0.080000000000 4.870846883557
0.090000000000 4.871524266835
0.100000000000 4.872281115422
0.110000000000 4.873117353863
0.120000000000 4.874032898845
0.130000000000 4.875027659218
0.140000000000 4.876101536027
0.150000000000 4.877254422539
0.160000000000 4.878486204275
0.170000000000 4.879796759043
0.180000000000 4.881185956978
0.190000000000 4.882653660577
0.200000000000 4.884199724740
0.210000000000 4.885823996817
0.220000000000 4.887526316647
0.230000000000 4.889306516611
0.240000000000 4.891164421680
0.250000000000 4.893099849462
0.260000000000 4.895112610264
0.270000000000 4.897202507140
0.280000000000 4.899369335954
0.290000000000 4.901612885438
0.300000000000 4.903932937252
0.310000000000 4.906329266045
0.320000000000 4.908801639541
0.330000000000 4.911349818575
0.340000000000 4.913973557184
0.350000000000 4.916672602670
0.360000000000 4.919446695671
0.370000000000 4.922295570255
0.380000000000 4.925218953967
0.390000000000 4.928216567925
0.400000000000 4.931288126898
0.410000000000 4.934433339393
0.420000000000 4.937651907702
0.430000000000 4.940943528045
0.440000000000 4.944307890603
0.450000000000 4.947744679660
0.460000000000 4.951253573632
0.470000000000 4.954834245189
0.480000000000 4.958486361375
0.490000000000 4.962209583585
0.500000000000 4.966003567821
0.510000000000 4.969867964682
0.520000000000 4.973802419487
0.530000000000 4.977806572371
0.540000000000 4.981880058384
0.550000000000 4.986022507590
0.560000000000 4.990233545168
0.570000000000 4.994512791514
0.580000000000 4.998859862341
0.590000000000 5.003274368783
0.600000000000 5.007755917529
0.610000000000 5.012304110814
0.620000000000 5.016918546688
0.630000000000 5.021598819017
0.640000000000 5.026344517612
0.650000000000 5.031155228340
0.660000000000 5.036030533229
0.670000000000 5.040970010578
0.680000000000 5.045973235061
0.690000000000 5.051039777842
0.700000000000 5.056169206680
0.710000000000 5.061361086039
0.720000000000 5.066614977199
0.730000000000 5.071930438364
0.740000000000 5.077307024773
0.750000000000 5.082744288810
0.760000000000 5.088241780114
0.770000000000 5.093799045688
0.780000000000 5.099415630013
0.790000000000 5.105091075151
0.800000000000 5.110824920862
0.810000000000 5.116616704710
0.820000000000 5.122465962172
0.830000000000 5.128372226747
0.840000000000 5.134335030075
0.850000000000 5.140353902028
0.860000000000 5.146428370829
0.870000000000 5.152557963160
0.880000000000 5.158742204266
0.890000000000 5.164980618065
0.900000000000 5.171272727251
0.910000000000 5.177618053522
0.920000000000 5.184016117248
0.930000000000 5.190466438163
0.940000000000 5.196968535125
0.950000000000 5.203521926292
0.960000000000 5.210126129226
0.970000000000 5.216780660992
0.980000000000 5.223485038260
0.990000000000 5.230238777408

